Linear Complementarity Algorithms for Infinite Games

The performance of two pivoting algorithms, due to Lemke and Cottle and Dantzig, is studied on linear complementarity problems (LCPs) that arise from infinite games, such as parity, average-reward, and discounted games. The algorithms have not been previously studied in the context of infinite games, and they offer alternatives to the classical strategy-improvement algorithms. The two algorithms are described purely in terms of discounted games, thus bypassing the reduction from the games to LCPs, and hence facilitating a better understanding of the algorithms when applied to games. A family of parity games is given, on which both algorithms run in exponential time, indicating that in the worst case they perform no better for parity, average-reward, or discounted games than they do for general P-matrix LCPs.

==> conclusion.tex <==
\section{Future Work}

%\paragraph{Conclusions.}

%This paper shows that two natural, yet previously not considered,  
%algorithms for solving parity, average-reward, and discounted
%games run in exponential time in the worst case. 
%The algorithms, although new in the context of infinite games, are
%derived from the well-known pivoting algorithms due to Lemke, and Cottle
%and Dantzig for the LCP, a fundamental problem in mathematical
%programming. 


%\paragraph{Future Work.}

%Our adaptation of Lemke's algorithm for solving discounted games
%corresponds to its implementation in which the unit covering vector is
%used~\cite{CPS92}. 
%Randomizing the covering vector may exhibit better performance and
%should be considered. 
%Our proof that Lemke's algorithm takes exponential time in the worst
%case relies on a very specific choice of the initial strategy.
%The expected running time should be analyzed for a random initial
%strategy. 

%The worst-case analysis of the Cottle-Dantzig algorithm requires
%a careful choice of the order on vertices. 
%Future work should include the analysis of the expected running time
%for randomly chosen vertex orderings.

Our adaptation of Lemke's algorithm for solving discounted games corresponds to
its implementation in which the unit covering vector is used~\cite{CPS92}, and
our lower bounds are specific to this choice. Similarly our lower bounds for the
Cottle-Dantzig algorithm require a specific choice of ordering over the
vertices. Randomizing these choices may exhibit better performance and should be
considered.

Adler and Megiddo~\cite{AM85} studied the performance of Lemke's algorithm for
the LCPs arising from linear programming problems.  They showed that, for
randomly chosen linear programs and a carefully selected covering vector, the
expected number of pivots performed by the algorithm is quadratic.  A similar
analysis for randomly chosen discounted games should be considered. 

